Decentralized Entropic Optimal Transport for Distributed Distribution Comparison

Distributed distribution comparison aims to measure the distance between the distributions whose data are scattered across different agents in a distributed system and cannot even be shared directly among the agents. In this study, we propose a novel decentralized entropic optimal transport (DEOT) method, which provides a communication-efficient and privacy-preserving solution to this problem with theoretical guarantees. In particular, we design a mini-batch randomized block-coordinate descent (MRBCD) scheme to optimize the DEOT distance in its dual form. The dual variables are scattered across different agents and updated locally and iteratively with limited communications among partial agents. The kernel matrix involved in the gradients of the dual variables is estimated by a decentralized kernel approximation method, in which each agent only needs to approximate and store a sub-kernel matrix by one-shot communication and without sharing raw data. Besides computing entropic Wasserstein distance, we show that the proposed MRBCD scheme and kernel approximation method also apply to entropic Gromov-Wasserstein distance. We analyze our method's communication complexity and, under mild assumptions, provide a theoretical bound for the approximation error caused by the convergence error, the estimated kernel, and the mismatch between the storage and communication protocols. In addition, we discuss the trade-off between the precision of the EOT distance and the strength of privacy protection when implementing our method. Experiments on synthetic data and real-world distributed domain adaptation tasks demonstrate the effectiveness of our method.

==> sections-arxiv/theory.tex <==
\section{Theoretical analysis}\label{sec:theory}
For the proposed decentralized entropic optimal transport method, we need to analyze and measure the quality of the guaranteed approximated solution.
First, because of the mismatch between storage and communication protocols, the gap between $\widetilde{W}_{\varepsilon}(\mu,\gamma)$ and ${W}_{\varepsilon}(\mu,\gamma)$ can be denoted as the {\em{model error}}.
Let $F_{\varepsilon}\left( u,v; K \right)$ and $\widetilde{F}_{\varepsilon}\left( u,v; K \right)$ denote the dual function value of \eqref{eq:dual-eot} and \eqref{eq:sample-eot} respectively with {\color{red}{real kernel}} $K$.
The model error can be written as
$$e_{model} = \left| \widetilde{F}_{\varepsilon}\big( \widetilde{u}^{*},\widetilde{v}^{*}; K \big) - F_{\varepsilon}\big( u^{*},v^{*}; K \big) \right|,$$where $\widetilde{u}^*$ and $\widetilde{v}^*$ denote the optimal solution of problem~\ref{eq:sample-eot}; $u^{*}$ and $v^{*}$ denote the optimal solution of original problem~\ref{eq:dual-eot}.
The {\em{model error}} has been discussed in Theorem~\ref{thm:approx_error}.
Further, before calculating the approximate distance $\widetilde{W}_{\varepsilon}(\mu,\gamma)$ through \eqref{eq:sample-eot}, the privacy-preserved kernel approximation scheme is employed to decentralized estimate kernel matrix $K$ with $\widehat{K}$.
This gap can be denoted as the {\em{kernel approximation error}}, i.e.,
$$e_{kernel} = \left| \widetilde{F}_{\varepsilon}\big( \widehat{u}^{*},\widehat{v}^{*}; \widehat{K} \big) - \widetilde{F}_{\varepsilon}\big( \widetilde{u}^{*},\widetilde{v}^{*}; K \big) \right|,$$where $\widehat{u}^*$ and $\widehat{v}^*$ denote the optimal solution of problem~\ref{eq:sample-eot} with approximate kernel $\widehat{K}$.
The {\em{kernel approximation error}} has been partly discussed in Theorem~\ref{thm:kernel-approx} with kernel gap result between $K$ and $\widehat{K}$.
According to \cite{dempe2015lipschitz}[Lemma 3.1] and \cite{bonnans2013perturbation}, it can be obtained that the perturbation on problem parameter $K$ can determine the change of the optimal objective value.
The following result can be obtained, i.e.,
\begin{eqnarray}\label{eq:kernel-error}
\!\!\!\!\!\!e_{kernel} \!\!\!\!&\le&\!\!\!\! L_{kernel} \cdot \big\| \widehat{K} - K \big\| \\
\!\!\!\!\!\!\!\!\!\!\!\!&\le&\!\!\!\! {\textstyle{L_{kernel}GN\Bigl( \sqrt{\frac{32\pi^2}{P}\log\frac{2N}{\delta}} + \frac{8\pi}{3P}\log\frac{2N}{\delta} \Bigr),}}\nonumber
\end{eqnarray}where $L_{kernel}$ in \eqref{eq:kernel-error} can be considered as the Lipschitz constant of the optimal value function $\widetilde{F}_{\varepsilon}$ with kernel $K$ as a parameter.
The detailed proof of \eqref{eq:kernel-error} can be found in Appendix~\ref{appendix:kernel error}.
The second inequality is obtained by Theorem~\ref{thm:kernel-approx}.


Finally, the proposed DRBCD method aims to optimize the approximate problem \eqref{eq:sample-eot} with the approximate kernel $\widehat{K}$, which also leads to the {\em{algorithm error}}, i.e.,
$$e_{algorithm} (u^t,v^t) = \left| \widetilde{F}_{\varepsilon}\big( u^t,v^t; \widehat{K} \big) - \widetilde{F}_{\varepsilon}\big( \widehat{u}^{*},\widehat{v}^{*}; \widehat{K} \big) \right|,$$where $u^t$ and $v^t$ denote the $t$-th iterates of the proposed method. 
The proposed {\color{red}{DRBCD}} method essentially can be considered as the decentralized and mini-batch stochastic implementation of typical randomized block coordinate descent method (RBCD)~\cite{nesterov2012efficiency,richtarik2014iteration,lu2015complexity} which has been popularly utilized to solve large-scale optimization problems.
In each iteration, the agent pairs are randomly chosen with the corresponding parameters to be updated (step 5 in Algorithm 2).
In addition, mini-batch stochastic scheme is employed to further enhance efficiency (steps 6 and 7 in Algorithm 2).
Let
$$\textstyle{{\cal{R}}_0:=\min_{\left( \widehat{u}^*,\widehat{v}^* \right)\in \widehat{\cal{W}}^*}\left\| \left(u^0,v^0\right) - \left( \widehat{u}^*,\widehat{v}^* \right)\right\|,}$$which measures the distance between the initial points $u^0,v^0$ and the optimal solution set $\widehat{\cal{W}}^*$ of \eqref{eq:sample-eot} with the approximate kernel $\widehat{K}$.
Further we assume the gradient norm can be bounded, i.e., $\left\| \nabla F_{\varepsilon} \right\|_2\le {\cal{R}}$.
Following the convergence and iteration complexity theoretical results in~\cite{wang2014randomized}[Theorem 3], the following results can be established on the algorithm error.
\begin{lemma}\label{le:algorithm-error}
Let $\left\{ \left( u^t,v^t \right) \right\}$ be the sequence generated by the {\color{red}{DRBCD}} method, and 
$$
\textstyle{\widehat{u}^{t} = \frac{1}{t} \sum_{\ell=1}^{t} u^{\ell}, \quad \widehat{u}^{t} = \frac{1}{t} \sum_{\ell=1}^{t} u^{\ell}.}
$$Then the iterate $\left( u^t,v^t \right)$ satisfies
\begin{equation}\label{eq:convergence-theorem}
{\mathbb{E}} \left[ e_{algorithm} ({\color{red}{\widehat{u}^t,\widehat{v}^t}}) \right] \le {\cal{O}} \big( \frac{ \big(\sqrt{t} + L\big){\cal{R}}_0^2 + \sqrt{t} {\cal{R}}^2 }{t} \big),
\end{equation} where the expectation is calculated with respect to the randomly selected agents and it also indicates the theoretical bound of the algorithm error.
\end{lemma}

Overall, we can establish the following error bound discussion with respect to our proposed model and method, which means that we need to analyze the performance of the obtained solutions.
We first define the gap between the obtained solution of the approximate model and the optimal solution of original model, i.e.,
$$
e_{all} (u,v) := \big| \widetilde{F}_{\varepsilon} \big( u,v; \widehat{K} \big) - F_{\varepsilon} \big( u^{*},v^{*}; K \big)  \big|.
$$The overall error can be further analyzed based the above model error, the kernel approximation error and the algorithm error.
For $\big( u^t,v^t \big)$, we have that
\begin{eqnarray}
\!\!\!\!\!\!\!\!&&\!\!\!\! e_{all} (u^t,v^t) := \big| \widetilde{F}_{\varepsilon} \big( u^t,v^t; \widehat{K} \big) - F_{\varepsilon} \big( u^{*},v^{*}; K \big)  \big| \nonumber \\
\!\!\!\!\!\!\!\!&\le &\!\!\!\! \big| \widetilde{F}_{\varepsilon} \big( u^k,v^k; \widehat{K} \big) - \widetilde{F}_{\varepsilon} \big( \widehat{u}^{*},\widehat{v}^{*}; \widehat{K} \big) \big| + \big| \widetilde{F}_{\varepsilon} \big( \widehat{u}^{*}, \widehat{v}^{*}; \widehat{K} \big) \nonumber\\
\!\!\!\!\!\!\!\!&&\!\!\!\! -\widetilde{F}_{\varepsilon} \big( \widetilde{u}^{*}, \widetilde{v}^{*}; K \big)  \big| + \big| \widetilde{F}_{\varepsilon} \big( \widetilde{u}^{*},\widetilde{v}^{*}; K \big) - F_{\varepsilon} \big( u^{*},v^{*}; K \big) \big| \nonumber \\
\!\!\!\!\!\!\!\!& = &\!\!\!\! e_{algorithm} \big( u^t,v^t \big) + e_{kernel} + e_{model}.
\end{eqnarray}
To summarize, the overall error is determined by all the above discussed errors, i.e., the model error, the kernel approximation error, and the algorithm error.

